On the analysis of scheduling algorithms for structured parallel computations

Algorithms for scheduling structured parallel computations have been widely studied in the literature. For some time now, Work Stealing is one of the most popular for scheduling such computations, and its performance has been studied in both theory and practice. Although it delivers provably good performances, the effectiveness of its underlying load balancing strategy is known to be limited for certain classes of computations, particularly the ones exhibiting irregular parallelism (e.g. depth first searches). Many studies have addressed this limitation from a purely load balancing perspective, viewing computations as sets of independent tasks, and then analyzing the expected amount of work attached to each processor as the execution progresses. However, these studies make strong assumptions regarding work generation which, despite being standard from a queuing theory perspective --- where work generation can be assumed to follow some random distribution --- do not match the reality of structured parallel computations --- where the work generation is not random, only depending on the structure of a computation. In this paper, we introduce a formal framework for studying the performance of structured computation schedulers, define a criterion that is appropriate for measuring their performance, and present a methodology for analyzing the performance of randomized schedulers. We demonstrate the convenience of this methodology by using it to prove that the performance of Work Stealing is limited, and to analyze the performance of a Work Stealing and Spreading algorithm, which overcomes Work Stealing's limitation.

==> sections/2-preliminaries-stability-generalize-lemma-proof.tex <==
\begin{proof}[Proof of Lemma~\ref{lemma:stability-generalize}]
  First, recall that $R_{\overline{t}}$ is partitioned through the processors.
  By Requirement~\ref{requirement:node-execution-constraints}, $C_{\overline{t}}$ is also partitioned through the processors and $\forall p \in Procs$, $R_{\overline{t}}\left(p\right) \supseteq C_{\overline{t}} \left(p\right)$.
  Thus, \[\sum_{p \in S} \left|R_{\overline{t}}\left(p\right) - C_{\overline{t}}\left(p\right)\right| = \left|R_{\overline{t}}\left( S\right) - C_{\overline{t}}\left( S\right)\right|\]
  To conclude the proof, note that by the linearity of expectation, \[\sum_{p \in S}E\left[\left|R_{\overline{t+1}}\left(p\right) - C_{\overline{t+1}}\left(p\right)\right|\right] = E\left[\left|R_{\overline{t+1}}\left(S\right) - C_{\overline{t+1}}\left( S\right)\right|\right]\]
\end{proof}


==> sections/4-wss-algorithm-short-term-stability-proof.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                                                                                                                           %
%                                                                                                                                           %
%                                                                                                                                           %
%                                                       Worst case for p's donations                                                        %
%                                                                                                                                           %
%                                                                                                                                           %
%                                                                                                                                           %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

We now prove that the greater is the number of processors making steal, the smaller are the chances that $p$'s spread attempts succeeds.

\begin{lemma}
  \label{lemma:p-spread-attempt-probability-decreases-with-more-spreads}
  Let $spreads\left(p,\alpha,d\right)$ be a function corresponding to the expected number of nodes that $p$ spreads during any round, where the ratio of idle processors of the round is $\alpha$ and the number of processors enabling two nodes is $d$.
  Then, $spreads\left(p,\alpha,d\right) \geq spreads\left(p,\alpha,P\left(1-\alpha\right)\right)$.
\end{lemma}
\begin{proof}[Proof of Lemma~\ref{lemma:p-spread-attempt-probability-decreases-with-more-spreads}]
  If $p$ targets a processor whose \algid{state} flag is set to \textsc{working}, then its spread attempt fails.
  Thus, in this case $p$ would not spread a node, regardless of the number of processors that make a spread attempt.
  However, if $p$ targets a processor whose \algid{state} flag is set to \textsc{idle}, then its attempt has a chance to succeed.
  We now consider the two possible situations:
  \begin{description}[leftmargin=0cm,noitemsep,topsep=5pt,parsep=5pt,partopsep=0pt]
  \item[$d = P\left(1 - \alpha\right)$] --- In this case, $spreads\left(p,\alpha,d\right) = spreads\left(p,\alpha,P\left(1-\alpha\right)\right)$.
  \item[$d \neq P \left(1 - \alpha\right)$] --- By definition there are $P \left(1 - \alpha\right)$ busy processors, implying that $d \leq P \left(1 - \alpha\right)$.
    Thus, for this case we conclude $d < P \left(1 - \alpha\right)$.
    Now, suppose $p$ targets some processor $q$ whose \algid{state} flag is set to \textsc{idle}.
    Thanks to the synchronous environment we have artificially created, and assuming that any call to \algid{UniformlyRandomNumber} takes the same number of steps, then every processor executes the \algid{CAS} instruction --- whose success dictates the success of the spread attempt --- at the same step (line 30 of Algorithm~\ref{algo:wss}).
    Finally, as a consequence of our assumptions regarding the \algid{CAS} instruction (see the first paragraph of Section~\ref{sec:analyzing-wss}) and since processors target donees uniformly at random, the greater the number of spread attempts that target $q$ the smaller are the chances for $p$'s spread attempt to succeed, concluding the proof of this lemma.
  \end{description}
\end{proof}



\begin{lemma}
\label{lemma:bab-lower bounds on the expected non-empty bins for a fixed number of balls}
Suppose there are $B$ bins, each of which is painted either red or green, and let $B_{R}$ and $B_{G}$ denote the initial number of red and green bins, respectively.
Additionally, let $\alpha$ denote the initial ratio of red bins, meaning $\alpha = \frac{B_{R}}{B}$ and $B \left(1 - \alpha\right) = B_{G}$.
Now, suppose there are $B_{R}$ cubes and $B_{G}$ balls.
First, each cube is tossed, independently and uniformly at random, into the bins.
After tossing all the $B_{R}$ cubes, count the number of cubes that landed in green bins, and, for each such cube, a red bin is painted green.
After finishing all the paintings, each of the $B_{G}$ balls is tossed, independently and uniformly at random, into the bins.
\\
Let $Y$ denote the number of bins that are still red, with at least one ball.
Then, \[E\left[Y\right] \geq B \alpha^{2} \left(1 - \euler^{- \left(1 - \alpha\right)}\right).\]
\end{lemma}
\begin{proof}[Proof of Lemma~\ref{lemma:bab-lower bounds on the expected non-empty bins for a fixed number of balls}]
Let $C_{G hit}$ and $B_{R \mapsto G}$ be two random variables, corresponding, respectively, to the number of cubes that land in green bins and to the number of red bins that are painted green.
Then, $B_{R \mapsto G} = C_{G hit}$, and thus
\begin{align*}
  E\left[B_{R \mapsto G}\right] &= E\left[C_{G hit}\right] \\
                                &= B \alpha \left(1 - \alpha\right).
\end{align*}
%
Similarly to Lemma~\ref{lemma:bab-lower bounds on the probability that i is non-empty}, for a bin $b_{i}$ let $Y_{i}$ be an indicator variable, defined as \[Y_{i} = \left\{\begin{matrix}
 \,1 & \text{if at least one ball lands in } b_{i};\\
 \,0 & \text{otherwise.}
\end{matrix}\right.\]
Thus, the probability that none of the $B_{G}$ balls lands in $b_{i}$ is
\begin{align*}
  P\left\{Y_{i} = 0\right\} &= \left(1 - \frac{1}{B}\right)^{B\left(1 - \alpha\right)} \\
                            &\leq \euler^{- \left(1 - \alpha\right)}.
\end{align*}
%
Since the probability that no ball lands in $b_{i}$ is independent from the number of red bins painted green (\textit{i.e.}~$Y_{i}$ is independent from $B_{R \mapsto G}$), then, for any $m$,
\[P\left\{Y_{i} = 0 | B_{R \mapsto G} = m\right\} = P\left\{Y_{i} = 0\right\}, \quad \text{and,} \quad P\left\{Y_{i} = 1 | B_{R \mapsto G} = m\right\} = P\left\{Y_{i} = 1\right\}.\]
It follows
\begin{align*}
  E\left[Y_{i} | B_{R \mapsto G} = m\right] &= 0 . P\left\{Y_{i} = 0 | B_{R \mapsto G} = m\right\} + 1 . P\left\{Y_{i} = 1 | B_{R \mapsto G} = m\right\} \\
                                            &= P\left\{Y_{i} = 1\right\} \\
                                            &\geq 1 - \euler^{- \left(1 - \alpha\right)}.
\end{align*}
%
Consider \[Y = \sum_{i = 1}^{B_{R} - B_{R \mapsto G}} Y_{i},\] corresponding to the number of bins that are still red with at least one ball.
By the linearity of expectation, it follows
\begin{align*}
E\left[Y | B_{R \mapsto G} = m\right] &= E\left[Y_{1} + Y_{2} + \ldots + Y_{B_{R} - m} | B_{R \mapsto G} = m\right] \\
&= \sum_{i = 1}^{B_{R} - m} E\left[Y_{i} | B_{R \mapsto G} = m\right] \\
&\geq \sum_{i = 1}^{B_{R} - m} \left(1 - \euler^{- \left(1 - \alpha\right)}\right) \\
&= \left(B_{R} - m\right) \left(1 - \euler^{- \left(1 - \alpha\right)}\right). \\
\end{align*}
%
To conclude this proof, by the law of total expectation it follows
\begin{align*}
  E\left[Y\right] &= \sum_{m = 0}^{B_{R}} \left(E\left[Y | B_{R \mapsto G} = m\right] P\left\{B_{R \mapsto G} = m\right\}\right) \\
                  &\geq \sum_{m = 0}^{B_{R}} \left(\left(B_{R} - m\right) \left(1 - \euler^{- \left(1 - \alpha\right)}\right) P\left\{B_{R \mapsto G} = m\right\}\right) \\
                  &= \left(1 - \euler^{- \left(1 - \alpha\right)}\right) \sum_{m = 0}^{B_{R}} \left(\left(B_{R} - m\right) P\left\{B_{R \mapsto G} = m\right\}\right) \\
                  &= \left(1 - \euler^{- \left(1 - \alpha\right)}\right) \left(\sum_{m = 0}^{B_{R}} \left(B_{R} P\left\{B_{R \mapsto G} = m\right\}\right) - \sum_{m = 0}^{B_{R}} \left(m P\left\{B_{R \mapsto G} = m\right\}\right)\right) \\
                  &= \left(1 - \euler^{- \left(1 - \alpha\right)}\right) \left(B_{R} - E\left[B_{R \mapsto G}\right]\right) \\
                  &= \left(1 - \euler^{- \left(1 - \alpha\right)}\right) \left(B \alpha - B \left(1 - \alpha\right) \alpha\right) \\
                  &= B \alpha^{2} \left(1 - \euler^{- \left(1 - \alpha\right)}\right)
\end{align*}
\end{proof}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                                                                                                                           %
%                                                                                                                                           %
%                                                                                                                                           %
%                                                       Worst case for p's donations                                                        %
%                                                                                                                                           %
%                                                                                                                                           %
%                                                                                                                                           %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


We now obtain lower bounds on the total number of spreads (or donations) made to processors during the second phase of some scheduling iteration, assuming that all busy processors make a spread attempt.

\begin{lemma}
  \label{lemma:lower-bounds-total-number-of-spreads}
  Consider any round $\overline{t}$ during a computation's execution, and let $B_{\overline{t}}$ be the set of processors that are busy during $\overline{t}$.
  If $\forall p \in B_{\overline{t}}, \left|E_{\overline{t}}\left(p\right)\right| = 2$, then $\mathrm{E}\bracks{|Spread^{+}_{\overline{t}}\left(B_{\overline{t}}\right)|} \geq P \alpha_{\overline{t}}^{2} \left(1 - \euler^{- \left(1 - \alpha_{\overline{t}}\right)}\right)$.  
\end{lemma}

\begin{proof}[Proof of Lemma~\ref{lemma:lower-bounds-total-number-of-spreads}]
  We prove this result by making an analogy with Lemma~\ref{lemma:bab-lower bounds on the expected non-empty bins for a fixed number of balls}:
  \begin{enumerate*}
  \item the number of bins $B$ corresponds to the number of processors $P$;
  \item the initial ratio of red and green bins correspond, respectively, to the ratio of idle and busy processors during the round;
  \item each cube toss corresponds to a steal attempt;
  \item each red bin that is painted green corresponds to a processor that was idle but whose steal attempt succeeded, and thus changed its \algid{state} flag to \textsc{working}; and
  \item each ball toss corresponds to a spread attempt.
  \end{enumerate*}
  Note that we can make this analogy because all steal attempts (and consequent \algid{state} flag updates) take place during the first phase of scheduling iterations while all spread attempts take place during the second phase of scheduling iterations. 
  Thus, $\mathrm{E}\bracks{|Spread^{+}_{\overline{t}}\left(B_{\overline{t}}\right)|} \geq P \alpha_{\overline{t}}^{2} \left(1 - \euler^{- \left(1 - \alpha_{\overline{t}}\right)}\right)$.
\end{proof}

\begin{proof}[Proof of Lemma~\ref{lemma:lower-bounds-expected-spreads-p}]
  By Lemma~\ref{lemma:p-spread-attempt-probability-decreases-with-more-spreads} it follows that $\mathrm{E}\bracks{|Spread^{+}_{\overline{t}}\left(p_{\overline{t}}\right)|}$ is the smallest if all busy processors enabled two nodes, and thus made a spread attempt.
  By Lemma~\ref{lemma:lower-bounds-total-number-of-spreads}, the expected number of nodes spread during a round such that all busy processors make a spread attempt is at least $P \alpha_{\overline{t}}^{2} \left(1 - \euler^{- \left(1 - \alpha_{\overline{t}}\right)}\right)$.
  Since, as we already noted, all processors have the same chances to make a successful spread attempt, and because each spread attempt may migrate at most one node, it follows that the expected number of nodes spread by each processor that makes a spread attempt is the same.
  Thus, since the expected number of nodes that $p$ spreads is the smallest if all processors make a spread attempt, then, letting $B_{\overline{t}}$ denote the set of processors that are busy during $\overline{t}$, it follows
  \[\mathrm{E}\bracks{|Spread^{+}_{\overline{t}}\left(p_{\overline{t}}\right)|} = \frac{\mathrm{E}\bracks{|Spread^{+}_{\overline{t}}\left(B_{\overline{t}}\right)|}}{P(1 - \alpha_{\overline{t}})} \geq \frac{\alpha_{\overline{t}}^{2}}{1 - \alpha_{\overline{t}}} \left(1 - \euler^{- \left(1 - \alpha_{\overline{t}}\right)}\right).\]
\end{proof}



==> sections/4-wss-lower-bounds-spreads.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                                                                                                                           %
%                                                                                                                                           %
%                                                                                                                                           %
%                                                       Worst case for p's donations                                                        %
%                                                                                                                                           %
%                                                                                                                                           %
%                                                                                                                                           %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

We now prove that the greater is the number of processors making steal, the smaller are the chances that $p$'s spread attempts succeeds.

\begin{lemma}
  \label{lemma:p-spread-attempt-probability-decreases-with-more-spreads}
  Let $spreads\left(p,\alpha,d\right)$ be a function corresponding to the expected number of nodes that $p$ spreads during any round, where the ratio of idle processors of the round is $\alpha$ and the number of processors enabling two nodes is $d$.
  Then, $spreads\left(p,\alpha,d\right) \geq spreads\left(p,\alpha,P\left(1-\alpha\right)\right)$.
\end{lemma}
\begin{proof}[Proof of Lemma~\ref{lemma:p-spread-attempt-probability-decreases-with-more-spreads}]
  If $p$ targets a processor whose \algid{state} flag is set to \textsc{working}, then its spread attempt fails.
  Thus, in this case $p$ would not spread a node, regardless of the number of processors that make a spread attempt.
  However, if $p$ targets a processor whose \algid{state} flag is set to \textsc{idle}, then its attempt has a chance to succeed.
  We now consider the two possible situations:
  \begin{description}[leftmargin=0cm,noitemsep,topsep=5pt,parsep=5pt,partopsep=0pt]
  \item[$d = P\left(1 - \alpha\right)$] --- In this case, $spreads\left(p,\alpha,d\right) = spreads\left(p,\alpha,P\left(1-\alpha\right)\right)$.
  \item[$d \neq P \left(1 - \alpha\right)$] --- By definition there are $P \left(1 - \alpha\right)$ busy processors, implying that $d \leq P \left(1 - \alpha\right)$.
    Thus, for this case we conclude $d < P \left(1 - \alpha\right)$.
    Now, suppose $p$ targets some processor $q$ whose \algid{state} flag is set to \textsc{idle}.
    Thanks to the synchronous environment we have artificially created, and assuming that any call to \algid{UniformlyRandomNumber} takes the same number of steps, then every processor executes the \algid{CAS} instruction --- whose success dictates the success of the spread attempt --- at the same step (line 30 of Algorithm~\ref{algo:wss}).
    Finally, as a consequence of our assumptions regarding the \algid{CAS} instruction (see the first paragraph of Section~\ref{sec:analyzing-wss}) and since processors target donees uniformly at random, the greater the number of spread attempts that target $q$ the smaller are the chances for $p$'s spread attempt to succeed, concluding the proof of this lemma.
  \end{description}
\end{proof}



\begin{lemma}
\label{lemma:bab-lower bounds on the expected non-empty bins for a fixed number of balls}
Suppose there are $B$ bins, each of which is painted either red or green, and let $B_{R}$ and $B_{G}$ denote the initial number of red and green bins, respectively.
Additionally, let $\alpha$ denote the initial ratio of red bins, meaning $\alpha = \frac{B_{R}}{B}$ and $B \left(1 - \alpha\right) = B_{G}$.
Now, suppose there are $B_{R}$ cubes and $B_{G}$ balls.
First, each cube is tossed, independently and uniformly at random, into the bins.
After tossing all the $B_{R}$ cubes, count the number of cubes that landed in green bins, and, for each such cube, a red bin is painted green.
After finishing all the paintings, each of the $B_{G}$ balls is tossed, independently and uniformly at random, into the bins.
\\
Let $Y$ denote the number of bins that are still red, with at least one ball.
Then, \[E\left[Y\right] \geq B \alpha^{2} \left(1 - \euler^{- \left(1 - \alpha\right)}\right).\]
\end{lemma}
\begin{proof}[Proof of Lemma~\ref{lemma:bab-lower bounds on the expected non-empty bins for a fixed number of balls}]
Let $C_{G hit}$ and $B_{R \mapsto G}$ be two random variables, corresponding, respectively, to the number of cubes that land in green bins and to the number of red bins that are painted green.
Then, $B_{R \mapsto G} = C_{G hit}$, and thus
\begin{align*}
  E\left[B_{R \mapsto G}\right] &= E\left[C_{G hit}\right] \\
                                &= B \alpha \left(1 - \alpha\right).
\end{align*}
%
Similarly to Lemma~\ref{lemma:bab-lower bounds on the probability that i is non-empty}, for a bin $b_{i}$ let $Y_{i}$ be an indicator variable, defined as \[Y_{i} = \left\{\begin{matrix}
 \,1 & \text{if at least one ball lands in } b_{i};\\
 \,0 & \text{otherwise.}
\end{matrix}\right.\]
Thus, the probability that none of the $B_{G}$ balls lands in $b_{i}$ is
\begin{align*}
  P\left\{Y_{i} = 0\right\} &= \left(1 - \frac{1}{B}\right)^{B\left(1 - \alpha\right)} \\
                            &\leq \euler^{- \left(1 - \alpha\right)}.
\end{align*}
%
Since the probability that no ball lands in $b_{i}$ is independent from the number of red bins painted green (\textit{i.e.}~$Y_{i}$ is independent from $B_{R \mapsto G}$), then, for any $m$,
\[P\left\{Y_{i} = 0 | B_{R \mapsto G} = m\right\} = P\left\{Y_{i} = 0\right\}, \quad \text{and,} \quad P\left\{Y_{i} = 1 | B_{R \mapsto G} = m\right\} = P\left\{Y_{i} = 1\right\}.\]
It follows
\begin{align*}
  E\left[Y_{i} | B_{R \mapsto G} = m\right] &= 0 . P\left\{Y_{i} = 0 | B_{R \mapsto G} = m\right\} + 1 . P\left\{Y_{i} = 1 | B_{R \mapsto G} = m\right\} \\
                                            &= P\left\{Y_{i} = 1\right\} \\
                                            &\geq 1 - \euler^{- \left(1 - \alpha\right)}.
\end{align*}
%
Consider \[Y = \sum_{i = 1}^{B_{R} - B_{R \mapsto G}} Y_{i},\] corresponding to the number of bins that are still red with at least one ball.
By the linearity of expectation, it follows
\begin{align*}
E\left[Y | B_{R \mapsto G} = m\right] &= E\left[Y_{1} + Y_{2} + \ldots + Y_{B_{R} - m} | B_{R \mapsto G} = m\right] \\
&= \sum_{i = 1}^{B_{R} - m} E\left[Y_{i} | B_{R \mapsto G} = m\right] \\
&\geq \sum_{i = 1}^{B_{R} - m} \left(1 - \euler^{- \left(1 - \alpha\right)}\right) \\
&= \left(B_{R} - m\right) \left(1 - \euler^{- \left(1 - \alpha\right)}\right). \\
\end{align*}
%
To conclude this proof, by the law of total expectation it follows
\begin{align*}
  E\left[Y\right] &= \sum_{m = 0}^{B_{R}} \left(E\left[Y | B_{R \mapsto G} = m\right] P\left\{B_{R \mapsto G} = m\right\}\right) \\
                  &\geq \sum_{m = 0}^{B_{R}} \left(\left(B_{R} - m\right) \left(1 - \euler^{- \left(1 - \alpha\right)}\right) P\left\{B_{R \mapsto G} = m\right\}\right) \\
                  &= \left(1 - \euler^{- \left(1 - \alpha\right)}\right) \sum_{m = 0}^{B_{R}} \left(\left(B_{R} - m\right) P\left\{B_{R \mapsto G} = m\right\}\right) \\
                  &= \left(1 - \euler^{- \left(1 - \alpha\right)}\right) \left(\sum_{m = 0}^{B_{R}} \left(B_{R} P\left\{B_{R \mapsto G} = m\right\}\right) - \sum_{m = 0}^{B_{R}} \left(m P\left\{B_{R \mapsto G} = m\right\}\right)\right) \\
                  &= \left(1 - \euler^{- \left(1 - \alpha\right)}\right) \left(B_{R} - E\left[B_{R \mapsto G}\right]\right) \\
                  &= \left(1 - \euler^{- \left(1 - \alpha\right)}\right) \left(B \alpha - B \left(1 - \alpha\right) \alpha\right) \\
                  &= B \alpha^{2} \left(1 - \euler^{- \left(1 - \alpha\right)}\right)
\end{align*}
\end{proof}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                                                                                                                           %
%                                                                                                                                           %
%                                                                                                                                           %
%                                                       Worst case for p's donations                                                        %
%                                                                                                                                           %
%                                                                                                                                           %
%                                                                                                                                           %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


We now obtain lower bounds on the total number of spreads (or donations) made to processors during the second phase of some scheduling iteration, assuming that all busy processors make a spread attempt.

\begin{lemma}
  \label{lemma:lower-bounds-total-number-of-spreads}
  Consider any round $\overline{t}$ during a computation's execution, and let $B_{\overline{t}}$ be the set of processors that are busy during $\overline{t}$.
  If $\forall p \in B_{\overline{t}}, \left|E_{\overline{t}}\left(p\right)\right| = 2$, then $\mathrm{E}\bracks{|Spread^{+}_{\overline{t}}\left(B_{\overline{t}}\right)|} \geq P \alpha_{\overline{t}}^{2} \left(1 - \euler^{- \left(1 - \alpha_{\overline{t}}\right)}\right)$.  
\end{lemma}

\begin{proof}[Proof of Lemma~\ref{lemma:lower-bounds-total-number-of-spreads}]
  We prove this result by making an analogy with Lemma~\ref{lemma:bab-lower bounds on the expected non-empty bins for a fixed number of balls}:
  \begin{enumerate*}
  \item the number of bins $B$ corresponds to the number of processors $P$;
  \item the initial ratio of red and green bins correspond, respectively, to the ratio of idle and busy processors during the round;
  \item each cube toss corresponds to a steal attempt;
  \item each red bin that is painted green corresponds to a processor that was idle but whose steal attempt succeeded, and thus changed its \algid{state} flag to \textsc{working}; and
  \item each ball toss corresponds to a spread attempt.
  \end{enumerate*}
  Note that we can make this analogy because all steal attempts (and consequent \algid{state} flag updates) take place during the first phase of scheduling iterations while all spread attempts take place during the second phase of scheduling iterations. 
  Thus, $\mathrm{E}\bracks{|Spread^{+}_{\overline{t}}\left(B_{\overline{t}}\right)|} \geq P \alpha_{\overline{t}}^{2} \left(1 - \euler^{- \left(1 - \alpha_{\overline{t}}\right)}\right)$.
\end{proof}

\begin{proof}[Proof of Lemma~\ref{lemma:lower-bounds-expected-spreads-p}]
  By Lemma~\ref{lemma:p-spread-attempt-probability-decreases-with-more-spreads} it follows that $\mathrm{E}\bracks{|Spread^{+}_{\overline{t}}\left(p_{\overline{t}}\right)|}$ is the smallest if all busy processors enabled two nodes, and thus made a spread attempt.
  By Lemma~\ref{lemma:lower-bounds-total-number-of-spreads}, the expected number of nodes spread during a round such that all busy processors make a spread attempt is at least $P \alpha_{\overline{t}}^{2} \left(1 - \euler^{- \left(1 - \alpha_{\overline{t}}\right)}\right)$.
  Since, as we already noted, all processors have the same chances to make a successful spread attempt, and because each spread attempt may migrate at most one node, it follows that the expected number of nodes spread by each processor that makes a spread attempt is the same.
  Thus, since the expected number of nodes that $p$ spreads is the smallest if all processors make a spread attempt, then, letting $B_{\overline{t}}$ denote the set of processors that are busy during $\overline{t}$, it follows
  \[\mathrm{E}\bracks{|Spread^{+}_{\overline{t}}\left(p_{\overline{t}}\right)|} = \frac{\mathrm{E}\bracks{|Spread^{+}_{\overline{t}}\left(B_{\overline{t}}\right)|}}{P(1 - \alpha_{\overline{t}})} \geq \frac{\alpha_{\overline{t}}^{2}}{1 - \alpha_{\overline{t}}} \left(1 - \euler^{- \left(1 - \alpha_{\overline{t}}\right)}\right).\]
\end{proof}


